On the Sensitivity of Deflagrations in Chandrasekhar Mass White Dwarf to Initial Conditions

We analyze the sensitivity of the flame propagation in a Chandrasekhar mass white dwarf to initial conditions during the subsonic burning phase, using 2D simulations of the full WD. Results are presented for a wide variety of initial flame distributions including central and off-center single point and multi-point, simultaneous and non-simultaneous, ignitions. We also examine the effects of convective velocity field which should exist at the core before the thermo-nuclear runaway. Our main conclusion suggests that the amounts of burning products and their distributions through the deflagration phase are extremely sensitive to initial conditions, much more sensitive than presented in previous studies. In particular, we find that more complex configurations such as even slight off-center ignitions, non-simultaneous multi-point ignitions and velocity fields tend to favor solutions in which individual plumes rise faster than the bulk of a typical Rayleigh-Taylor driven, unstable burning front. The difference to previous calculations for an octant of a WD may be understood as a consequence of the suppression of l=1,2 modes. Our results are consistent with full star calculations by the Chicago group. Moreover, the total amount of nuclear burning during the phase of subsonic burning depends sensitively on the initial conditions and may cause the WD to pulsate or to become unbound. We discuss the implications of the results on current models for Type Ia SNe, limitations imposed by the 2-D nature of our study, and suggest directions for further study.

==> dir_apj/README <==
% README -- Contents of the AASTeX macro package distribution

Thanks for your interest in the AASTeX macros for manuscript preparation.
This directory contains all the files in the distribution.  They are
described briefly immediately below.  Following the file descriptions
are short installation instructions, the generic recipe for printing the
user guide and samples, and information about contacting us regarding
the distribution.


README			This file
RelNotes.v40            Release Notes for v4.0.
Changes                 Summary of all package revisions.

aasms4.doc		Fully documented source for the "manuscript"
			substyle.  Contains macro definitions + comments.
aasms4.sty		LaTeX input style file for the "manuscript"
			substyle.  This is the .doc file stripped of
			comments and unnecessary whitespace.

aaspp4.doc		Fully documented source for the "preprint"
			substyle.  Contains macro definitions + comments.
aaspp4.sty		LaTeX input style file for the "preprint"
			substyle.  This is the .doc file stripped of
			comments and unnecessary whitespace.

aas2pp4.doc		Documented source for a two-column preprint substyle.
aas2pp4.sty		LaTeX input style file for two-column preprint
			substyle.

amssym.sty              LaTeX input style file for AMS fonts v2.1 definitions.

aj_pt4.doc		Documented source for the AJ plano tables substyle.
aj_pt4.sty		LaTeX input style file for AJ plano tables substyle.

apjpt4.doc		Documented source for the ApJ plano tables substyle.
apjpt4.sty		LaTeX input style file for ApJ plano tables substyle.

art8.doc		Documented 8pt style option.
art8.sty		LaTeX input style file for the 8pt style option.

eqsecnum.sty		Substyle file that enables equations to be
			numbered with sections, rather than ordinally.

epsf.sty		A copy of Rokicki's epsf.sty file that is supplied
			with dvips.  It is included so that style files
			can be interpreted, and so that authors can
			include proper space for EPS files even if they
			do not have dvips.

flushrt.sty             Style file that enables full justification and 
                          hyphenation.

tighten.sty             Substyle definition for "single-spaced" manuscripts

aastex.tex		The user guide for the package.

ams.ps                  PostScript paper containing lists of AMS fonts that 
                          may be used with AASTeX.

sample1.tex		Minimal sample paper.
sample2.tex		Sample paper with "typical" content and markup.
samp2tbl.tex	        "Long" table for sample2.tex, marked up as a camera-
			  ready (plano) table.

complext.tex            Short but complex plano table.

samptbls.tex		More plano table samples.  Sets style and includes:
table1.tex		  Sample plano table #1.
table2.tex		  Sample plano table #2.
table3.tex		  Sample plano table #3.

graphics.tex		Initial proposal to WGAS and Pubs Board
			suggesting standardized use of Encapsulated
			PostScript for graphics inclusions.
sgi*.eps		Encapsulated PostScript plots for graphics.tex and
                          sample2.tex.

kspp.tex		Preprint format proposal from K.Sellgren to the
			Pubs Board.

aastex40.tar.Z		All of the above files can be retrieved at once
			in this compressed tarfile, if desired.


INSTALLING THE STYLE FILES

The *.sty files must be "installed" so that LaTeX can read them.  This
simply means that they must be placed either in (1) the user's working
directory containing the paper being processed [single-user installation],
or (2) in the TeX/LaTeX system input directory [site-wide installation].

Individuals who obtain the files for their personal use should just put
the files in the same directory that they usually use when preparing
papers, memos, etc., with LaTeX.

Sites that expect usage by several authors will probably find it preferable
to install the files in the standard TeX inputs area.  In the parlances of
popular OS's, these areas are typically called

	/usr/local/lib/tex/inputs	Unix and variants
	SOME$DISK:[TEX.INPUTS]		VMS/Files-11 specification
	C:\EMTEX\TEXINPUT		DOS

The *.doc files are not actually read by LaTeX.  They are the "source code"
files for the corresponding .sty files.  The *.sty files are produced
mechanically from the *.doc files; these .sty files are never edited.
Most installations of LaTeX keep .doc and .sty files in the same directory
so that they can be easily found.  We suggest doing the same with these.

The user's guide and sample papers could be kept in a system-wide TeX
inputs directory as well, but the system administrator may find it desirable
to change the filenames somewhat, since they are quite generic and prone
to filename collisions.


PRINTING THE GUIDE AND SAMPLES

The User Guide should be printed out for best results in reading it.
The Guide is written using the aaspp substyle from the AASTeX macro
package, and is therefore a LaTeX document.  It must be processed by
LaTeX, resulting in a compiled, device-independent format (a .dvi file).
The DVI file has to be translated through a program that knows about the
specific printer you wish to print on; such a program is often called a
"DVI driver".

Suppose you wish to print on a PostScript laser printer, and that the
DVI driver on your computer system is called "dvips".  The generic steps
to be followed to get hardcopy are

    prompt> latex aastex
    prompt> dvips aastex
    prompt> print aastex.ps

There are various system- and program-specific eccentricities which
cannot be fully enumerated here.  Some things to watch out for:

    1.  On some systems, TeX and LaTeX do not permit a filename extension
	(the .tex) on the input file specification; .tex is assumed.
	On other systems, it is optional.
    2.  Most DVI drivers do not require the .dvi extension on the input
	filename.  The extension of the output file (the one destined
	for a specific printer) is variable, often a site-dependent
	configuration parameter.
    3.  The user interfaces for DVI drivers are quite inconsistent.
	Some operate in an interactive mode, asking the user about
	variable setup parameters, while some only accept control
	input on the command line.
    4.  On some systems, the DVI translation and printing are combined,
	so one would enter only one OS command after running LaTeX.

There is no way for us to know details of your installation, so you must
inquire of the system administrator responsible for LaTeX, or hope that
someone has written the LaTeX "Local Guide" for your site.


ADMINISTRATIVE DETAILS

This package has been prepared by Chris Biemesderfer on behalf of the
AAS Executive Office.  It has evolved from a project of the Working
Group on Astronomical Software (WGAS), chaired by Bob Hanisch of the
Space Telescope Science Institute in Baltimore.  We would like to
express appreciation to the National Radio Astronomy Observatory and
National Optical Astronomy Observatories for their support of this
project during its germination.

Comments, suggestions, complaints, etc., can be sent electronically.
Community feedback is valuable, and will be retained and evaluated so
that we can coordinate the evolution of the package with the
requirements of editors and publishers as moderated by the AAS
Executive Office and the Publications Board.

Chris Biemesderfer 7 Jan 1993
revised 20 Apr 1995


AASTeX Support:  aastex-help@aas.org


